reSolve - A Transverse Momentum Resummation Tool

In this note, we introduce the new tool reSolve, a Monte Carlo differential cross-section and parton-level event generator whose main purpose is to add transverse momentum resummation to a general class of inclusive processes at hadron colliders, namely all those which do not involve hadrons or jets in the measured final state. This documentation refers to the first main version release, which will form the basis for continued developments, consequently it only implements the key features of those we plan to ultimately include. This article acts as a manual for the program; describing in detail its use, structure, validation and results; whilst also highlighting key aspects of the resummation formalism applied. It details the two classes of processes so far included; these are diphoton production and Drell-Yan production. A main concept behind the development of the tool is that it is a hands-on white box for the user: significant effort has been made to give the program a modular structure, making the various parts which comprise it independent of each other as much as possible and ensuring they are transparently documented, customizable and, in principle, replaceable with something that may better serve the users needs. reSolve is a new C++ program, based on an evolution of the private Fortran code 2gres, previously used for the calculations in refs. [1] and [2]; it is also influenced by the DYRes Fortran code of refs. [3] and [4]. This initial version calculates the low transverse momentum contribution to the fully differential cross-section for two main categories of processes; the inclusive production of two photons, and inclusive Drell-Yan production. In all cases resummation up to Next-to-Next-to-Leading Logarithm (NNLL) is included. We aim to extend the program to several more processes in the near future. The program is publicly available on Github.

==> Figure data/Figure 18/gnuplot_plotting_qT_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qTplot_reSolve_revamp_NNLO_test1.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.30]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/reSolve_NNLO_test1_histo_0_qT.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/2gres_NNLO_test1_histo_0_qT.dat" u 1:2:4 w yerr notitle lw 1 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/reSolve_NNLO_test1_histo_0_qT.dat" u 1:2 w lines t "reSolve" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/2gres_NNLO_test1_histo_0_qT.dat" u 1:2 w lines lw 3 lt 1 lc 14 title "2gres"


==> Figure data/Figure 18/gnuplot_plotting_qq_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qqplot_reSolve_revamp_NNLO_test1.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.20]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/reSolve_NNLO_test1_histo_0_qq.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/2gres_NNLO_test1_histo_0_qq.dat" u 1:2:4 w yerr notitle lw 1 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/reSolve_NNLO_test1_histo_0_qq.dat" u 1:2 w lines t "reSolve" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 18/2gres_NNLO_test1_histo_0_qq.dat" u 1:2 w lines lw 3 lt 1 lc 14 title "2gres"


==> Figure data/Figure 19/gnuplot_plotting_qT_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qTplot_reSolve_revamp_NNLO_test2.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.12]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/reSolve_NNLO_test2_qT.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/2gres_NNLO_test2_qT.dat" u 1:2:4 w yerr notitle lw 1 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/reSolve_NNLO_test2_qT.dat" u 1:2 w lines t "reSolve" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/2gres_NNLO_test2_qT.dat" u 1:2 w lines lw 3 lt 1 lc 14 title "2gres"


==> Figure data/Figure 19/gnuplot_plotting_qq_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qqplot_reSolve_revamp_NNLO_test2.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.10]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/reSolve_NNLO_test2_qq.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/2gres_NNLO_test2_qq.dat" u 1:2:4 w yerr notitle lw 1 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/reSolve_NNLO_test2_qq.dat" u 1:2 w lines t "reSolve" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 19/2gres_NNLO_test2_qq.dat" u 1:2 w lines lw 3 lt 1 lc 14 title "2gres"


==> Figure data/Figure 20/gnuplot_plotting_script_100_bins <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qqplot_reSolve_test1_100bins.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.20]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 20/reSolve_NNLO_test1_qq_100bins.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 20/reSolve_NNLO_test1_qq_100bins.dat" u 1:2 w lines t "reSolve 100 bins" lw 3 lt 1 lc 2


==> Figure data/Figure 20/gnuplot_plotting_script_200_bins <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qqplot_reSolve_test1_200bins.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.20]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 20/reSolve_NNLO_test1_qq_200bins.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 4, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 20/reSolve_NNLO_test1_qq_200bins.dat" u 1:2 w lines t "reSolve 200 bins" lw 3 lt 1 lc 4


==> Figure data/Figure 20/gnuplot_plotting_script_50_bins <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qqplot_reSolve_test1_50bins.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.20]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 20/reSolve_NNLO_test1_qq_50bins.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 20/reSolve_NNLO_test1_qq_50bins.dat" u 1:2 w lines t "reSolve 50 bins" lw 3 lt 1 lc 1


==> Figure data/Figure 21/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qqplot_Atlas_A_reSolveand2gres.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:500]
set yrange [0:0.1]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 21/reSolve_Atlas_A_histo_1_qq_160bins.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 21/2gres_Atlas_A_histo_1_qq.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 21/reSolve_Atlas_A_histo_1_qq_160bins.dat" u 1:2 w lines t "reSolve" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 21/2gres_Atlas_A_histo_1_qq.dat" u 1:2 w lines lw 3 lt 1 lc 14 title "2gres"




==> Figure data/Figure 22/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qTplot_Atlas_A_reSolveand2gres.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.3]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 22/reSolve_Atlas_A_histo_0_qT_100bins.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 22/2gres_Atlas_A_histo_0_qT.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 22/reSolve_Atlas_A_histo_0_qT_100bins.dat" u 1:2 w lines t "reSolve" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 22/2gres_Atlas_A_histo_0_qT.dat" u 1:2 w lines lw 3 lt 1 lc 14 title "2gres"




==> Figure data/Figure 23/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/qTplot_reSolve_revamp_Atlas_witherrors.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.50]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 23/pTspec_reSolve_revamp_Atlas_withscalevarandmontecarlo.dat" u 1:2 w lines notitle lw 3 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 23/pTspec_reSolve_revamp_Atlas_withscalevarandmontecarlo.dat" u 1:5 w lines notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 23/pTspec_reSolve_revamp_Atlas_withscalevarandmontecarlo.dat" u 1:7 w lines notitle lw 3 lt 1 lc 2,"/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 23/pTspec_reSolve_revamp_Atlas_withscalevarandmontecarlo.dat" u 1:7:8 w yerr title "ATLAS" lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 23/pTspec_reSolve_revamp_Atlas_withscalevarandmontecarlo.dat" u 1:2:3:4 w yerr title "2gres" lw 3 lt 1 lc 14,"/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 23/pTspec_reSolve_revamp_Atlas_withscalevarandmontecarlo.dat" u 1:5:6 w yerr title "reSolve" lw 3 lt 1 lc 7



==> Figure data/Figure 24/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/yZ_qT_reSolveanddyres.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:170]
set yrange [-0.2:15]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 24/reSolve_histo_0_qT_NNLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 24/reSolve_histo_0_qT_NNLO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} NNLO(+NNLL)" lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 24/dyres_yZ_NNLO_qT.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 10, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 24/dyres_yZ_NNLO_qT.dat" u 1:2 w lines t "DYRes Z/{/Symbol g} NNLO(+NNLL)" lw 3 lt 1 lc 10


==> Figure data/Figure 25/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/yZ_eta_NNLO_reSolveanddyres.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/d{/Symbol h} (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "{/Symbol h}" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [-2:2]
set yrange [0:60]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 25/reSolve_yZ_histo_0_eta.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 25/reSolve_yZ_histo_0_eta.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} NNLO(+NNLL)" lw 3 lt 1 lc 7, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 25/dyres_yZ_NNLO_eta.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 14, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 25/dyres_yZ_NNLO_eta.dat" u 1:2 w lines t "DYRes Z/{/Symbol g} NNLO(+NNLL)" lw 3 lt 1 lc 14


==> Figure data/Figure 26/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/Z_qT_reSolveandDYRes.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:150]
set yrange [-0.2:150]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/reSolve_histo_0_qT_NNLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/reSolve_histo_0_qT_NNLO.dat" u 1:2 w lines t "reSolve Z onshell NNLO(+NNLL)" lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/dyres_NNLO_qT.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/dyres_NNLO_qT.dat" u 1:2 w lines t "DYRes Z onshell NNLO(+NNLL)" lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/reSolve_histo_0_qT_NLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/reSolve_histo_0_qT_NLO.dat" u 1:2 w lines t "reSolve Z onshell NLO(+NLL)" lw 3 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/dyres_NLO_qT.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 4, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 26/dyres_NLO_qT.dat" u 1:2 w lines t "DYRes Z onshell NLO(+NLL)" lw 3 lt 1 lc 4


==> Figure data/Figure 27/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/yZ_pTmaxmin_multiplot_pbperGeV.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set yrange [-0.2:30.0]
### Start multiplot (2x2 layout)
set multiplot layout 1,2 rowsfirst
# Margins for each row resp. column
LMARGIN = "set lmargin at screen 0.15; set rmargin at screen 0.55"
RMARGIN = "set lmargin at screen 0.55; set rmargin at screen 0.95"
# --- GRAPH a
set label 1 '(a)' at graph 0.05,0.95 font ',24'
set xlabel "pTmin (GeV)" font ",28" offset 0,0,0
set xrange [15:85]
@LMARGIN
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmin_absolutepbperGeV_NLO.dat" u 1:2 w lines notitle lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmin_absolutepbperGeV_NLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmin_absolutepbperGeV_NLO.dat" u 1:2 w lines notitle lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmin_absolutepbperGeV_NNLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmin_absolutepbperGeV_NNLO.dat" u 1:2 w lines notitle lw 2 lt 1 lc 1
# --- GRAPH b
set label 1 '(b)' at graph 0.01,0.95 font ',24'
set xlabel "pTmax (GeV)" font ",28" offset 0,0,0
set xrange [15:85]
@RMARGIN
set format y ''; unset ylabel
set key at graph 1, 1 box opaque
set key width 1.1
set key height 1
set key font ", 18"
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmax_absolutepbperGeV_NLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmax_absolutepbperGeV_NLO.dat" u 1:2 w lines t "Z/{/Symbol g} NLO(+NLL)" lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmax_absolutepbperGeV_NNLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 27/histo_0_pTmax_absolutepbperGeV_NNLO.dat" u 1:2 w lines t "Z/{/Symbol g} NNLO(+NNLL)" lw 2 lt 1 lc 1
unset multiplot
### End multiplot



==> Figure data/Figure 28/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/Z_eta_absolute.eps'
set grid
#set title "eta histogram" font ",36"
set ylabel "d{/Symbol s}/d{/Symbol h} (pb/bin)" font ",28" offset 0,0,0
set xlabel "{/Symbol h}" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [-5:5]
set yrange [0:80.0]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 28/histo_0_absolute_eta_NNLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 28/histo_0_absolute_eta_NNLO.dat" u 1:2 w lines t "reSolve Z Onshell NNLO(+NNLL)" lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 28/histo_0_absolute_eta_NLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 28/histo_0_absolute_eta_NLO.dat" u 1:2 w lines t "reSolve Z Onshell NLO(+NLL)" lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 28/histo_0_absolute_eta_LO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 28/histo_0_absolute_eta_LO.dat" u 1:2 w lines t "reSolve Z Onshell LO" lw 3 lt 1 lc 3


==> Figure data/Figure 29/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/Wpm_mT.eps'
set grid
#set title "mT histogram" font ",36"
set ylabel "d{/Symbol s}/dm_T (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "m_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [20:100]
set yrange [0:120.0]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 29/histo_0_mT_NNLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 29/histo_0_mT_NNLO.dat" u 1:2 w lines t "reSolve W+- NNLO(+NNLL)" lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 29/histo_0_mT_NLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 29/histo_0_mT_NLO.dat" u 1:2 w lines t "reSolve W+- NLO(+NLL)" lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 29/histo_0_mT_LO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 29/histo_0_mT_LO.dat" u 1:2 w lines t "reSolve W+- LO" lw 3 lt 1 lc 3


==> Figure data/Figure 30/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/yZ_qq.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:150]
set yrange [0:40]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 30/histo_0_qq_NNLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 30/histo_0_qq_NNLO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} NNLO(+NNLL)" lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 30/histo_0_qq_NLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 30/histo_0_qq_NLO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} NLO(+NLL)" lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 30/histo_0_qq_LO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 30/histo_0_qq_LO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} LO" lw 3 lt 1 lc 3


==> Figure data/Figure 31/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/Wpm_qT.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:80]
set yrange [-1:200.0]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 31/histo_0_qT_NNLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 31/histo_0_qT_NNLO.dat" u 1:2 w lines t "reSolve W+- NNLO(+NNLL)" lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 31/histo_0_qT_NLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 31/histo_0_qT_NLO.dat" u 1:2 w lines t "reSolve W+- NLO(+NLL)" lw 2 lt 1 lc 2


==> Figure data/Figure 32/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/Wpm_eta.eps'
set grid
#set title "eta histogram" font ",36"
set ylabel "d{/Symbol s}/d{/Symbol h} (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "{/Symbol h}" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [-4:4]
set yrange [0:600.0]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 32/histo_0_eta_NNLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 32/histo_0_eta_NNLO.dat" u 1:2 w lines t "reSolve W+- NNLO(+NNLL)" lw 3 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 32/histo_0_eta_NLO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 32/histo_0_eta_NLO.dat" u 1:2 w lines t "reSolve W+- NLO(+NLL)" lw 3 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 32/histo_0_eta_LO.dat" u 1:2:4 w yerr notitle lw 3 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 32/histo_0_eta_LO.dat" u 1:2 w lines t "reSolve W+- LO" lw 3 lt 1 lc 3


==> Figure data/Figure 33/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/yZ_mT.eps'
set grid
#set title "mT histogram" font ",36"
set ylabel "d{/Symbol s}/dm_T (pb/binwidth)" font ",28" offset 0,0,0
set xlabel "m_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:200]
set yrange [0:10]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 33/histo_0_mT_NNLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 33/histo_0_mT_NNLO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} NNLO(+NNLL)" lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 33/histo_0_mT_NLO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 33/histo_0_mT_NLO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} NLO(+NLL)" lw 2 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 33/histo_0_mT_LO.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 33/histo_0_mT_LO.dat" u 1:2 w lines t "reSolve Z/{/Symbol g} LO" lw 2 lt 1 lc 3


==> Figure data/Figure 34/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/reSolve_NNLO_test1_124pdffits_qq.eps'
set grid
#set title "qq histogram" font ",36"
set ylabel "d{/Symbol s}/dqq (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "qq (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.20]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 34/reSolve_NNLO_test1_1pdffit_qq.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 34/reSolve_NNLO_test1_2pdffit_qq.dat" u 1:2:4 w yerr notitle lw 1 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 34/reSolve_NNLO_test1_4pdffit_qq.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 34/reSolve_NNLO_test1_1pdffit_qq.dat" u 1:2 w lines t "reSolve 1 pdffit" lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 34/reSolve_NNLO_test1_2pdffit_qq.dat" u 1:2 w lines lw 2 lt 1 lc 2 t "reSolve 2 pdffits", "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 34/reSolve_NNLO_test1_4pdffit_qq.dat" u 1:2 w lines t "reSolve 4 pdffits" lw 2 lt 1 lc 3


==> Figure data/Figure 35/gnuplot_plotting_script <==
reset
set terminal postscript eps color enhanced "Helvetica" 20
set output '/home/tom/Resummation_Work/New_Draft_Journal/reSolve_NNLO_test1_124pdffits_qT.eps'
set grid
#set title "qT histogram" font ",36"
set ylabel "d{/Symbol s}/dq_T (pb/binwidth)" font ",28" offset 2,0,0
set xlabel "q_T (GeV)" font ",28" offset 0,0,0
set ytics font ", 20"
set ytics font ", 20"
set xrange [0:180]
set yrange [0:0.30]
plot "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 35/reSolve_NNLO_test1_1pdffit_qT.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 35/reSolve_NNLO_test1_2pdffit_qT.dat" u 1:2:4 w yerr notitle lw 1 lt 1 lc 2, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 35/reSolve_NNLO_test1_4pdffit_qT.dat" u 1:2:4 w yerr notitle lw 2 lt 1 lc 3, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 35/reSolve_NNLO_test1_1pdffit_qT.dat" u 1:2 w lines t "reSolve 1 pdffit" lw 2 lt 1 lc 1, "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 35/reSolve_NNLO_test1_2pdffit_qT.dat" u 1:2 w lines lw 2 lt 1 lc 2 t "reSolve 2 pdffits", "/home/tom/Resummation_Work/New_Draft_Journal/Figure\ data/Figure\ 35/reSolve_NNLO_test1_4pdffit_qT.dat" u 1:2 w lines t "reSolve 4 pdffits" lw 2 lt 1 lc 3

